Adversarial Attack and Defense on Graph Data: A Survey

Deep neural networks (DNNs) have been widely applied to various applications, including image classification, text generation, audio recognition, and graph data analysis. However, recent studies have shown that DNNs are vulnerable to adversarial attacks. Though there are several works about adversarial attack and defense strategies on domains such as images and natural language processing, it is still difficult to directly transfer the learned knowledge to graph data due to its representation structure. Given the importance of graph analysis, an increasing number of studies over the past few years have attempted to analyze the robustness of machine learning models on graph data. Nevertheless, existing research considering adversarial behaviors on graph data often focuses on specific types of attacks with certain assumptions. In addition, each work proposes its own mathematical formulation, which makes the comparison among different methods difficult. Therefore, this review is intended to provide an overall landscape of more than 100 papers on adversarial attack and defense strategies for graph data, and establish a unified formulation encompassing most graph adversarial learning models. Moreover, we also compare different graph attacks and defenses along with their contributions and limitations, as well as summarize the evaluation metrics, datasets and future trends. We hope this survey can help fill the gap in the literature and facilitate further development of this promising new field.

==> sec07-sum.tex <==
% \section{Summaries: Attack and Defense on graph}  \label{sec:summary}


\subsection{Defense Summary}

In this section, we compare eight existing relevant papers in Table \ref{table:comparision}.
Then, we talk about the contributions and limitations of these works.
Finally, we will discuss the potential research opportunities in this area.

% \begin{table*}[tbh!]
% \label{table:comparision}
% \resizebox{7in}{!}{% 
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
%                   & Semi-supervised & Un-supervised & Graph Classification & Node Classification & Link Prediction & Transferable \\ \hline
% Dai et al.           &\checkmark                 &               &\checkmark                      &\checkmark                     &                 &\checkmark             \\ \hline
% Zugner et al.    &\checkmark                 &               &                      &\checkmark                     &                 &\checkmark             \\ \hline
% Chen et al.    &                 &\checkmark               &                      &                     &\checkmark                 &\checkmark             \\ \hline
% Chen and Sun et al.    &                 &\checkmark               &                      &\checkmark                     &\checkmark                 &\checkmark             \\ \hline
% ICLR 19-1 &                 &\checkmark               &                      &\checkmark                     &\checkmark                 &\checkmark             \\ \hline
% ICLR 19-2      &\checkmark                 &               &                      &\checkmark                     &                 &\checkmark             \\ \hline
% ICLR 19-3          &\checkmark                 &               &                      &\checkmark                     &                 &             \\ \hline
% \end{tabular}
% }
% \caption{Comparisons between existing papers}
% \end{table*}

\textbf{Contributions}
We summarize the unique contributions of each works in this part.
% important information covered in each works in the Table \ref{table:comparision}.
% It is not hard to see that most existing papers can do the adversarial attacks on node classification task.
Dai et al. \cite{dai2018adversarial} use the reinforcement learning approach to discover the adversarial attack,
which is the only approach that support black-box attack comparing to other works.
Z{\"u}gner et al. \cite{zugner2018adversarial} study adversarial graph samples with traditional machine learning
and deep learning. Meanwhile, they are the first and only group to discuss the adversarial attack on the attribute graph.
Chen et al. and Sun et al. \cite{chen2018link, sun2018data} mainly attack the link predication task with deep graph convolutional embedding model.
ICLR 19-1 tries to attack the node embedding which is used for different tasks, such as link predication and node classification.
ICLR 19-2 attacks the node classification by using meta-learning which solve the bi-level problem underlying training-time attacks.
This work shows that by using small graph perturbations consistently lead to a strong decrease in performance for GCN.
ICLR 19-3 proposes a greedy algorithm to find the edges and use GAN to generate the close feature space to attack the model.
It is one of most efficient way to find the good quality adversarial samples.

\textbf{Limitations}
The limitations of most current works are summarized below. 
Most existing works didn't give very clear strategies about the setting of the budget and distance
with reasonable explanations in real applications.
Different with other adversarial attacks, most modifications on graph are hardly tell by the human in real life.
To solve this problem, we give a more detailed discussion on perturbation and evaluation metrics in the paper.
Meanwhile, about graph imperceptible evaluation metrics, 
most papers \cite{bojchevski2019adversarial, chen2018link, dai2018adversarial} use one metric for attack,
but these adversarial samples could be found by other existing imperceptible evaluation metrics.
In this work, we list all existing evaluation metrics,
and recommend future adversarial samples imperceptible with most existing evaluation metrics.
% Otherwise, every adversarial sample won't be imperceptible, since it can be easily discovered under some existing imperceptible metrics. 
Another main issue is that different problem formulations.
%All of them are adversarial attack on graph data, but it is hardly to see the relations and differences between them. 
To solve this problem, we give the unified problem formulation for all existing works discussed in this survey.

\textbf{Future Direction}
Adversarial attack on graph data is a new and hot area,
and many research opportunities are summarized below:
1) Most graphs are attributed graph on node and edge in the real life. Currently, very few existing works well studied adversarial attack on attributed graph, e.g., heterogeneous information graph.
2) Some advanced ideas can be applied for generating the adversarial samples, e.g., homomorphism graph.
3) Various learning settings are not attacked yet, such as inductive learning on node classification task.
4) There is none defense system proposed for adversarial attack on graph data.
5) The main limitation of existing attack methods is that they do not consider various imperceptibility metrics into their attack models.
% Concise imperceptibility metrics are necessary in different tasks.
% Different imperceptibility measures are needed in different tasks and scenarios.
We believe that an accurate and explainable evaluation metric could help discover more adversarial examples created by current methods. In addition, different and multiple imperceptibility measures are needed in different tasks and scenarios.
6) Last but not the least, the distance of high quality adversarial samples are not well studied in this area.
%how to measure the significance of attack techniques on graph data is still an open question in this area.
